Dynamic Detection of Inefficient Data Mapping Patterns in Heterogeneous OpenMP Applications

With the growing prevalence of heterogeneous computing, CPUs are increasingly being paired with accelerators to achieve new levels of performance and energy efficiency. However, data movement between devices remains a significant bottleneck, complicating application development. Existing performance tools require considerable programmer intervention to diagnose and locate data transfer inefficiencies. To address this, we propose dynamic analysis techniques to detect and profile inefficient data transfer and allocation patterns in heterogeneous applications. We implemented these techniques into OMPDataPerf, which provides detailed traces of problematic data mappings, source code attribution, and assessments of optimization potential in heterogeneous OpenMP applications. OMPDataPerf uses the OpenMP Tools Interface (OMPT) and incurs only a 5 % geometric-mean runtime overhead.

==> 7_survey.tex <==
\section{OMPT Compiler and Runtime Support} \label{sec:survey}

The \emph{OpenMP Tools Interface} (OMPT) and its subsequent extension with the \emph{External Monitoring Interface} (EMI) callbacks in OpenMP 5.1 has seen varying levels of adoption across different compilers and their associated runtimes.
This section provides an overview of the current compiler support for target-related OMPT features, which aims to inform future strategies for tool development for heterogeneous OpenMP applications.
We investigate and compare compilers from prominent hardware vendors, including AMD, ARM, Intel, and NVIDIA, as well as compilers from the GNU and LLVM projects. 
To assess compiler support for OpenMP OMPT features, we conducted a comprehensive review of publicly available documentation and manuals, audited source code (when available), and conducted basic testing.

\subsection{Compilers/Runtimes Supporting OMPT with EMI Callbacks}

    \subsubsection{LLVM Clang/Flang}
    Clang \cite{llvm-clang}, the C/C++ frontend for LLVM \cite{lattner2004llvm, llvm}, provides one of the most complete OpenMP implementations, with Flang's \cite{llvm-f18} support rapidly developing.
    LLVM's \\ \texttt{libomptarget} runtime supports offloading to AMD and NVIDIA GPUs \cite{llvm-19-1-0-OpenMPSupport}. 
    LLVM first implemented OMPT tool initialization and non-target callbacks in 6.0.0 (March 2018) based on the early technical reports (\href{https://github.com/llvm/llvm-project/commit/82e94a593433f36734e2d34898d353a2ecb65b8b}{\texttt{82e94a}}, \href{https://github.com/llvm/llvm-project/commit/cab9cdc2ad8b1c40d99ac07c5a03b8061a7f3868}{\texttt{cab9cd}}, \href{https://github.com/llvm/llvm-project/commit/e1a04b4659a6cc7ef0f777622b38c3da3535b92d}{\texttt{e1a04b}}, \href{https://github.com/llvm/llvm-project/commit/489cdb783a0655ed2d2812a62fda220eb17574dd}{\texttt{489cdb}}) \cite{llvm-6-0-0-OpenMPSupport}.
    LLVM 8.0.0 (March 2019) finalized these features in accordance with the OpenMP 5.0 specification only a few months after its ratification (\href{https://github.com/llvm/llvm-project/commit/0e0d6cdd5862d7c5e28c542fa07d6fadd07f1628}{\texttt{0e0d6c}}, \href{https://github.com/llvm/llvm-project/commit/2b46d30fc7049fc5cc5b9f98df654509bb4d61a2}{\texttt{2b46d3}}).
    Despite Clang's support documentation \cite{llvm-17-0-1-OpenMPSupport, llvm-18-1-0-OpenMPSupport} not indicating compliant 5.0 OMPT callback and 5.1 EMI support until 18.1.0-rc1 (\href{https://github.com/llvm/llvm-project/commit/99ce17b71c41190cd82f4c5382910d71cb673abe}{\texttt{99ce17}}), these features were actually completed in 17.0.0-rc4 with the inclusion of \href{https://github.com/llvm/llvm-project/commit/7e68c9e5c27182b867c1602a1095395089d3039c}{\texttt{7e68c9}} followed by minor bug fixes \href{https://github.com/llvm/llvm-project/commit/4d5feafb9dc0d7e9b12b116f07307085687c2e3d}{\texttt{4d5fea}} and \href{https://github.com/llvm/llvm-project/commit/1d54dc2f75861295aeb99f480aed244dc5cedea5}{\texttt{1d54dc}}.

    \subsubsection{AMD Optimizing C/C++ and Fortran Compilers (AOCC)} \hspace{0pt}\\
    Highly optimized for AMD Zen-based processors, the October 2024 release of AOCC 5.0 \cite{amd-aocc}, is built on LLVM 17.0.1 and is the first version of AOCC to support target and EMI callbacks while prior versions only supported non-target callbacks \cite{amd-aocc-5-0-OpenMPSupport, amd-aocc-4-2-OpenMPSupport}.

    \subsubsection{AMD ROCm}
    ROCm \cite{amd-rocm} is an open-source software stack optimized for AMD GPUs, consisting of compilers, libraries, and tools.
    ROCm contains a downstream LLVM project with additional enhancements for AMD GPUs.
    Target callbacks support was added in 5.7.0 (\href{https://github.com/ROCm/llvm-project/commit/12e5b16d5fe1a003788190a3c102532d79a18e00}{\texttt{12e5b1}}), released September 2023 \cite{amd-rocm-5-7-0-OpenMPSupport}.
    Additionally, in 5.1.0 (\href{https://github.com/ROCm/llvm-project/commit/b999647daa8d1f141261fa99e69d01690437415c}{\texttt{b99964}}), released March 2022, AMD implemented the OMPT tracing interface, a feature not yet available in the latest upstream LLVM project as of writing \cite{amd-rocm-5-1-0-OpenMPSupport}.

    \subsubsection{AMD AOMP}
    AOMP \cite{amd-aomp} is an open-source LLVM-based compiler with improved support for OpenMP on Radeon GPUs.
    AOMP builds on top of, and releases are more frequent than ROCm LLVM.
    Version 14.0-1 (January 2022) implements the OMPT tracing interface \cite{amd-aomp-14-0-1-OpenMPSupport}.
    Version 17.0-3 (July 2023) provides target and EMI callbacks \cite{amd-aomp-17-0-3-OpenMPSupport}.

    \subsubsection{HPE Cray Compiling Environment (CCE)}
    CCE \cite{hpe-cce} provides the Cray Fortran and C/C++ compilers which use the \texttt{libcraymp} and \texttt{libcrayacc} runtimes which can be used as drop-in replacements for LLVM's \texttt{libomp} and \texttt{libomptarget} runtimes or GNU's \texttt{libgomp} runtime.
    The C/C++ compiler is LLVM-based and supports offloading to AMD and NVIDIA GPUs.
    The November 2020 release of CCE 11.0.0 introduced OMPT 5.0 support \cite{hpe-cce-11-0-enhancements}.
    EMI callbacks were implemented in CCE 16.0.0 (May 2023) \cite{sc23-openmp-bof}.

    \subsubsection{Intel oneAPI DPC++/C++ (ICX) and Fortran (IFX) Compilers}
    ICX/IFX are proprietary LLVM-based compilers that have had target and EMI callbacks since version 2023.2 (July 2023) and support offloading to Intel GPUs. Additional plugins can enable offloading to AMD and NVIDIA GPUs.
    Support continues through the latest stable release as of writing, version 2024.2 (June 2024), and is based on LLVM 19 development \cite{intel-icx-OpenMPSupport, intel-dpcpp-changelog}.

    \subsubsection{NVIDIA HPC SDK (NVHPC)}
    NVIDIA’s HPC SDK \cite{nvidia-hpc} provides a subset of OpenMP 5.0 features and can offload to NVIDIA GPUs.
    Support for OMPT callbacks was introduced in version 22.7 (July 2022) as stated in the compiler release notes, although the compiler documentation does not indicate OMPT or EMI callback support even in the latest 24.9 September 2024 release as of writing \cite{nvidia-hpc-22-7-OpenMPSupport, nvidia-hpc-24-9-OpenMPSupport}.
    We tested to confirm which features were functional.
    Unlike LLVM-based compilers, NVHPC requires (re)compiling your code with the { \tt -mp=ompt } flag in order for OMPT-based tools to be invoked.

\subsection{Compilers/Runtimes Supporting OMPT without EMI Callbacks}

    \subsubsection{Arm Compiler for Linux (ACfL)}
    ACfL \cite{arm-acfl} is an LLVM-based compiler with optimizations for 64-bit Armv8-A server-class processors.
    The latest release, 24.04, is based on LLVM 18 but has offloading support disabled \cite{arm-c-OpenMPSupport, arm-fortran-OpenMPSupport}.
    Only non-target OMPT callbacks are supported.
    
\subsection{Compilers/Runtimes without OMPT Support}

    \subsubsection{GNU Compiler Collection (GCC)}
    The latest release of GCC \cite{gnu-gcc} as of writing, version 14.2, released August 2024, supports offloading to AMD and NVIDIA GPUs.
    However, GCC lacks support for OMPT entirely \cite{gnu-libgomp-14-2-OpenMPSupport}.
    This positions GCC behind LLVM-based compilers in terms of OpenMP tooling.





\subsection{Summary of OMPT Adoption Findings}

LLVM-based compilers, such as Clang/Flang, AMD AOCC/\hspace{0pt}ROCm/\hspace{0pt}AOMP, and Intel ICX/IFX, which closely track upstream LLVM developments, have mature, well-tested OMPT support that has seen steady and development to meet the latest OpenMP specifications.
NVIDIA's HPC SDK also achieves a high level of OMPT support and has target related OMPT features, a year prior to LLVM-based compilers.
Although Arm ACfL is based on LLVM, it does not have support for target offloading enabled.
However, it does include non-target-related OMPT support.
GNU GCC is the only compiler infrastructure we found that lacks OMPT support altogether.
Table \ref{tab:ompt_support} compares and summarizes OMPT-related feature support across these compilers and indicates the earliest version we could determine to support each feature.
Additionally, the footnotes of Table \ref{tab:ompt_support} indicate each feature's status in later OpenMP standard revisions, whether each feature is required to be compliant, and whether \texttt{OMPDataPerf} depends on the feature.

\subsection{Recommendations}

Proper implementation documentation of OMPT features by compiler/runtime implementers remains needed.
Among the compilers we examined that claimed OMPT support, \emph{none} clearly and/or correctly specified which exact features (i.e. callbacks/tracing interface) they actually supported.
Additionally, AMD AOMP and ROCm, both based on the same LLVM branch, are the only compilers to support the OMPT tracing interface.
Upstreaming this feature into the mainline LLVM should be considered to promote broader adoption.

For tool designers, the target EMI callbacks, excluding the target map EMI callback, are well supported across runtimes.
If ensuring maximal tool runtime compatibility or support going forward is a priority, tool developers should limit their usage of OMPT target callbacks to the EMI callbacks, again excluding the optional map callback.
Although the non-EMI versions of the same callbacks are currently well supported, they have recently been deprecated in OpenMP 6.0 \cite{openmpSpec60}.




